The Cloud Needs a Reputation System

Today's cloud apps are built from many diverse services that are managed by different parties. At the same time, these parties, which consume and/or provide services, continue to rely on arcane static security and entitlements models. In this paper, we introduce Seit, an inter-tenant framework that manages the interactions between cloud services. Seit is a software-defined reputation-based framework. It consists of two primary components: (1) a set of integration and query interfaces that can be easily integrated into cloud and service providers' management stacks, and (2) a controller that maintains reputation information using a mechanism that is adaptive to the highly dynamic environment of the cloud. We have fully implemented Seit, and integrated it into an SDN controller, a load balancer, a cloud service broker, an intrusion detection system, and a monitoring framework. We evaluate the efficacy of Seit using both an analytical model and a Mininet-based emulated environment. Our analytical model validate the isolation and stability properties of Seit. Using our emulated environment, we show that Seit can provide improved security by isolating malicious tenants, reduced costs by adapting the infrastructure without compromising security, and increased revenues for high quality service providers by enabling reputation to impact discovery.

==> Makefile <==
BUILD_DIR = .
OUTPUTDIR_OPTION = --output-directory $(BUILD_DIR)
SRC_FILES = ibm.bib refs.bib Seit2014.tex \
			abstract.tex \
			intro.tex \
			related.tex \
			motivation.tex \
			arch.tex \
			policiesandinterfaces.tex \
			ibr.tex \
			properties.tex \
			deployment.tex \
			impl.tex \
			eval.tex \
			discussion.tex 


FIGURES_DIR = Figures

all: Seit2014.pdf

Seit2014.pdf: $(SRC_FILES) $(FIGURES_DIR) 
	@if [ ! -d "$(BUILD_DIR)" ]; then mkdir -p $(BUILD_DIR); fi
	@-pdflatex $(OUTPUTDIR_OPTION) Seit2014.tex
	@-bibtex $(BUILD_DIR)/Seit2014
	@pdflatex $(OUTPUTDIR_OPTION) Seit2014.tex
	@pdflatex $(OUTPUTDIR_OPTION) Seit2014.tex

.PHONY: clean
clean:
	@cd $(BUILD_DIR) && rm -f *.aux *.bbl *.blg *.dvi *.log *.pdf *.ps


==> approach.tex <==
\section{Seit Approach}
Our goal in this paper is to address the challenges from the previous section without affecting 
the performance or the quality of service of tenants' applications. Our solution, Seit, provides an automotive high efficient system to classify tenants traffics and reroute them based on the receiver tenant requirements. Seit provides an automatic system to dynamically manage and control inter-tenant traffic in two steps (Automatic Tenant classification followed by Automatic tenant’s traffic routing) as described next.

\subsection {Automatic Tenant Classification}
 In the current version of Seit, we focus on classifying tenants based on their behavior although we envision the classification can be accomplished with other matrices such as tenant’s location, ownership, applications. We mean by behavior here is the intention of the tenant to cause harm to other tenants or the cloud datacenter. This harm can be, for example, DOS, DDOS, sending malicious traffic, overwhelming the victim’s network and resources, and unauthorized access to datacenter or other tenants’ resources. 

\begin{figure}[h]
\centering
	\includegraphics[width=\columnwidth, height=10cm]{graphs/IBR.pdf}
	\caption{IBR}
	\label{fig:batteryLog}
\end{figure}

To detect bad behaviors in efficient and quick manner, we implemented Introduction Based Routing (IBR) approach used in P2P systems. With IBR, peers are giving the choices with whom they interact with by providing incorporating feedback, giving participants a basis for making their relationship choices. IBR is decentralized system and requires minimum information sharing among peers and designed to scale to Internet sized networks with no modifications to operating systems and network backbone. To better understand IBR, consider the following example showing in figure[]. Nodes A, B, C and D are peers in P2P system. The green lines indicate established connections. Each node maintains reputation score for the nodes connected to it. When Node A wants to communicate with D, it must follow the chain of connections between it and D and ask the nodes in the chain for introduction to the node after. A starts asking B for introduction to C. Node B looks at node’s A behavior history (represented by reputation score AB) and decides whether or not to forward A’s request to C. If the request is forwarded, C looks at behavior history of B (BC) and decides whether or not to accept the introduction request. The process continues until A reaches D. If B, C, or D rejects a request, node A will not be able to communicate with D. After the connection is established between A and C, C assigns a reputations score to A (CA) which is X*BC. Same thing with D where it assigns reputations score of DA which is X* DC. If A starts behaving bad (e.g. sending malicious packets to D), D will decrease A’s score DA and also decreases C’s score DC since C took the responsibility and introduced A to D. C will do the same and decrease A’s score AC and B’s score since it introduced A to C. And finally, B will decrease A’s reputation score AB.  By this approach, nodes take extra cautious of whom they introduce and eventually, bad behaving nodes will be left alone with no other nodes willing to introduce them when their scores fall under the minimum accepted score.

In Seit, we used the same approach but on a tenant level. Since tenants own more than one host in the datacenter, they are responsible for their host’s behaviors and any miss behaving hosts will affect the tenant’s reputation. Moreover, although we could make Seit’s reputation system be completely decentralized, we decided to take advantage of the existing of a centralized management entity in the cloud to better provide IBR system with more robust implementation. When tenants detect bad behaviors, not only they will make decision of future introduction acceptance, but also inform the Cloud Manage CM of this behavior. This information helps CM to get a wide view of his datacenter and tenant sharing its resources and their overall behaviors which lead to make valuable decisions applied to tenant (isolating bad tenants, blocking their traffic, etc.).  Further, in traditional IBR in P2P networks, nodes perform hill-climbing algorithm, where hosts advertise nodes they accept introductions from to other nodes. Instead, we make tenant advertise node the accept introduction to only CM where it can calculate the shortest/best path and return the paths to all tenants. We believe by involving CM in our system, we could save the tenants the extra overhead and delay caused by searching and discovering introduction path to destination (especially in large datacenters with thousands of tenants in it). 

\subsection {Automatic Traffic Differentiate Routing}
Once tenants are classified based on their behaviors, we could easily classify and route their traffic by simply implementing SDN. When one of the tenant’s host (source) starts communicating with a host (destination) that belongs to another tenant (after introduction), Seit looks at source’s reputation score and matches the routing decision for destination (next section). Right after that, Seit informs the Openflow controller with these information (source IP, destination IP, protocol, action, etc.) so the controller can apply the appropriate rule for the traffic between the two hosts.

\subsection {Scoring system}

\begin{table}
\begin{center}
\caption{Tenant Score Table}
\begin{tabular}{|  p{1.2cm} |  p{1.4cm} |  p{1.4cm} | p{1.4cm} |}
  \hline                       
  Score - Application) & Mail & Web Server & CDN \\
  \hline
  0.0 - 0.1 & Block & Block & Block\\
  \hline
  0.1 - 0.2 & Block & Block & Forward to IDS\\
  \hline 
  0.2 - 0.5 & Block & Forward to IDS & Forward to IDS\\
  \hline
  0.5 - 0.8 & Forward to IDS & Forward to Proxy & Forward to IDS\\
  \hline
 0.8 - 1.0 & Forward to IDS & Allow & Allow\\
  \hline
\end{tabular}
\label{tab:waspMsgs}
\end{center}
%\label{tab:waspMsgs} %% Please do not revert this -- the reference is broken if placed here
\end{table}

The uniqueness of Seit that tenants are the ones who decide the traffic classification and how it is handled. Table [] shows an example of one of the tenants’ scoring system. Tenants provide the information of how traffic is handled for different score levels to variety of applications (or destination in their network) since different application might have different sensitivity. [] For example, tenant X requests that all incoming traffics to it from bad behaving tenants should be rerouted to IDS and all incoming traffics to it from good behaving tenants should be allowed to reach its destination directly. Tenant X does not have to classify the incoming traffic for a certain tenant (although it can do this in Seit). The classification will be applied to any tenant that wants to connect to tenant X. If tenant Y is communicating with tenant X and changes its behavior from good to bad (e.g sends malicious packets to tenant X), Seit system will automatically change the handling of the traffic and make flow through IDS. By this mechanism, there will be no need for manual configuration of the network and MBs.   


==> background.tex <==
\section{Background}
\subsection{P2P Reputation Systems}
\subsection{Tenant Behaviors}
\subsection{Impact of Attacks on Tenants}
\subsection{Flow Classifications}

==> deployment.tex <==
%\section{Deployment Model}
%
%In this section we illustrate how tenants within Seit's framework interact.
%\subsection{Seit's interaction with tenants}
%Figure \ref{fig:Seit-high-level} shows Seit's interaction with tenants. More text to illustrate....
%\begin{figure*}
		%\centering
        %\includegraphics[width=\textwidth]{graphs/Seit-High-level.pdf}
        %\caption{Seit High Level}
        %\label{fig:Seit-high-level}
%\end{figure*}
%\subsection{Accessing services} 
%Tenants that use Seit's framework should not be involved nor control how Seit builds their reputation. In other word, once the sensors and executors are configured (through their Seit interfaces), a tenant should provide and access services from other tenants as he used to do without Seit's framework. For example, if a tenant needs to connect his web service to an external database service from another tenant. All what he needs to do is specifying the external service's URL in his web services. The web service (under the hood) will send to Seit's engine a request to establish connection with the external service. Seit's engine then performs all the necessary introduction requests and returns with the external service's reputation score to the tenant's executors. The executers at this point execute the actions that map to the reputation received (e.g. open ports). At the same time, the tenant Web service (and any other sensors the tenant own) will keep updating its Seit engine of any feedback about the connection to the external service. Seit's engine, after receiving the feedback, update the reputation score of the other tenant and instruct the executors to execute the appropriate new actions that match the new reputation. 
%
%\subsection{Joining Seit's network and building reputation}
%When a tenant joins Seit's framework, it receives a default global reputation score (assigned by Reputation Manager) and zero local reputation since it did not start a connection with any tenant. In addition, since a tenant cannot see Seit's reputation system interaction (e.g. who is introducing to who), this will provide a good incentive and notion to be good and provide good service to as many other tenants as possible since it will affect its reputation eventually across all tenants. That also means if a tenant is planning to harm another one, it cannot figure out the chain to reach the target. 
%The speed to build a reputation depends on several factors such as number of tenants to interact with, QoF provided to these tenants, and any privacy and security threats to these tenants. 
%
%


==> discussion.tex <==
\section{Discussion}
In this section we explore and discuss some aspects of Seit.
\subsection{Using IBR}
We used Introduction Based Routing because of what it can provide of an interesting model of reputation and how it can increase and decrease through introductions. However, we do not claim any contribution on P2P area and we refrain from discussing the gaming aspect of as it is out of the scope of this paper. In addition, Seit engine can use other reputation systems such as (give other examples). At the end, all what the tenant needs is the reputation score of other tenants it interacts with to apply the appropriate actions toward them. 
 
\subsection{Overhead of establishing connection}
As we showed in this paper, tenants using Seit's framework can only communicate with each other after their Seit's engines establish the connection. We understand that this approach may present an extra delay compared to systems with no Seit's framework. But we believe the overhead is very small (test how long it takes) and only when engines establish the connection. Once the services start communicating, all the traffic should take the normal time.

\subsection{Role of Reputation Manager}
Reputation Manager (CM) is only an addition to Seit and not an essential component of it. We implemented the Reputation Manager component and its interface in our current system for the benefits it can provide to Seit's framework. However, we understand that in some situation we will not be able to use it. In other word, Seit should be able to work in an environment without the need to rely on CM. For example, if we have tenants that interact through Seit system in Amazon, we cannot force Amazon to install a Reputation Manager but the tenants in it should be able to interact as any P2P system.

\subsection{Complexity of configuring Seit's executors and sensors}
How do we scale especially with VMs? And how to make sure that policies among components don't conflict.

\subsection{Tenant that do not use Seit framework}
One of the benefits of Seit's framework that tenants who use it can interact with the ones who do not without any conflict. Each Seit tenant has the ability to choose which tenants to interact with individually and based on their reputation. It can also choose to interact with non Seit tenants and assign them the reputation that fit them most. We assume that if a tenant decides not to use Seit's framework and decides to interact with tenant that do, this tenant will always gets the least reputation as it will be risky to trust it.

\subsection{Symmetric of reputation and its reflection on QoS}
Asked by Carlee in her notes.
That’s a good point and worth more discussion. Peers don’t know their reputations at different neighbors. After Seit establishes a connection between two tenants and each knows the reputation score for the other, each tenant will inform the other of the QoS is should receive based on its score. For example. Let’s say we have two tenants, one is a web server and the other is SQL DB service. The SQL server agreed to provide the Web server with 5GB of space. Where the SQL account and data will be stored is not of the Web server concern. How it is traffic is being monitored through IDS of FW is not of its concern. All what it cares about that it gets 5GB and connection to the database. If for any reason the SQL service shuts down its database or doesn’t provide 5GB then the Web server will decrees the SQL service’s reputation score. 

==> goals.tex <==
\section{Design Goals}
\label{sec:goals}

Reputation systems have been used in peer-to-peer systems to prevent leachers (cites?), and in person-to-person communication
systems to prevent unwanted communication (OSTRA).  Applying to the cloud has the unique challenges in being
machine to machine, highly variable, and highly dynamic.  Here we highlight design goals toward addressing these challenges.


%% After motivated need for reputation system
\subsection{Local Reputation for Machine-to-Machine Communication}

Need reputation system for machine-to-machine which reflects individual tenant views.
different tenants interact differently
different tenants have different views of what is `bad'

and which can be stable, while still being dynamically (and automatically) adjustable

and which can effectively cluster tenants into groups (e.g., isolate bad tenants)


% OSTRA person to person, but shared other features

\subsection{Programmable Network Infrastructure}

Need API for tenants to be able to influence the infrastructure / how traffic is handled
toward a more efficient infrastructure (meaning cost, QoS, etc.).
Sec -- haproxy to send traffic to A (trusted clients) or B (untrusted clients)
Tenant Performance/cost -- bypass IDS (less VMs needed, so lower cost, and performance is increased since one less box to traverse)
Cloud Provider performance / cost -- e..g, blocking at source (of cloud provider's network)

% OSTRA -- just block

\subsection{Programmable Sensing Infrastructure} 

Need ability to mark something as `bad', but in M2M, it is not necessarily binary (good or bad).

Need 

% OSTRA -- user did this and it was binary



==> old.tex <==
%%% FROM ABSTRACT.tex

%
%Cloud services are not created equal. Some are good, some are slow,
%some are buggy, and some are malicious. Today's apps are built from
%many services that are managed by different parties and
%tenants. Their developers must, in turn, reason about the
%effectiveness of each service, relying mostly on user-generated
%reviews and ratings. At the same time, services, which are consumed by
%many apps (or other services), continue to rely on arcane static
%security and entitlements models.
%
%Developers must reason about the
%effectiveness of each service, relying mostly on user-generated
%reviews and ratings. 


-------------------------------------------------------
%%% FROM MOTIVATION.tex


%Verizon. 2014 DATA BREACH INVESTIGATIONS REPORT
% External detection: 99% of point-of-sale intrusions, 88% for web apps with financial motive, 98% for web apps with idealollogy motive, 
% 68% for misc. error in data leakage, 45% in cases of insider misuse of data.


%2-	Motivational Examples
%a.	Host all trusted tenants in one server and the untrusted on other server to minimize risk
%b.	The incentive of  providing good service to good tenants 
%c.	Amount of resources saved (IBM Data Power)
%d.	HAProxy load balancing with IDS (picture)

%%A main goal of Seit is to use reputation to enable tenants or cloud providers
%%to be able to automatically adjust how traffic is handled toward a more 
%%secure and efficient infrastructure.  
%One might use reputation to separate clients on different
%sets of servers to give the trusted clients better security assurances, or use
%reputation to allow certain tenants to bypass middleboxes (decreasing cost for the 
%server tenant, and improving performance for the client tenants that have good 
%reputation), or use reputation to block traffic from sources deemed 
%unwanted (decreasing traffic on the cloud providers network).
%While programmable components are widely available (via
%configuration), and research is proposing systems for easier
%interfacing (via provided APIs), the automatic management of them is
%lacking.  
%In Section~\ref{sec:cloudintegration}, we elaborate on how Seit can be 
%interfaced with components as well as how Seit supports the highly dynamic 
%nature of the cloud through an configurable query interface that provides
%support for efficient continuous query and feedback. 

-------------------------------------------------------
%%% FROM ARCH.tex

%%% Somewhere I want to talk about like where a tenant might not be malicious, but
%%% could be careless, which should have less reputation than a very careful tenant.

%Need ability to mark something as `bad', but in M2M, it is not necessarily binary (good or bad).
% OSTRA -- user did this and it was binary


%As shown in Figure \ref{fig:detailed-proc}, Seit framework architecture contains of three components: Seit Tenants, Reputation Manager, and Seit Messages.
%\subsection{Seit Tenant}
%A tenant Represents a group of VMs and services that belong and managed by a costumer, company, or department. In order for a tenant to be part of Seit framwork and take adventage of its interaction, it has to take the rule of three types as shown in Figure \ref{fig:intro-process}: \paragraphb{Requester} that request to establish a connection such as tenant A, \paragraphb{Introducer} that introduce tenants to each other such as tenant B, or \paragraphb{Target} such as tenant C where it receive introduction request from introducer tenants to establish connection with requester tenant. In addition. every tenant in Seit framework must contains the following entities:
%\begin{itemize}
%\item \paragraphb{Seit Engine (SE)} A component within a tenant's group and initially configured and managed by tenant. SE is responsible to exchange Inter-Tenant messages and establish connections with other SEs that belong to other tenants. JE also receives internal feedback from "Sensors" within tenant's group and external feedback from other tenants. SE, according to feedback received, instructs "Executors" to implement and execute "Actions" defined by the tenant. 
%
%\item \paragraphb{Sensors} Components within a tenant's group that sense and monitor a certain behavior (e.g traffic, services) and notify SE through "Seit Interface". Example of sensor are IDS and resource monitors, or service itself.
%
%\item \paragraphb{Executors} Components within tenant's group that receive and execute actions from SE through Seit Executor Plugin. For example an SDN controller that receives and executes Openflow rules as indicated by SE. Or a firewall that receives commands to block or allow certain traffic
%
%\item \paragraphb{Seit Interface (SI)} Executors and sensors within tenant install SI which has an API to communicate and receive actions commands from SE and map these commands to actual actions executors implement.
%\end{itemize}
%
%It is important to highlight that tenant's entities could be deployed as individual VMs, processors within one VM, or mix of both. For example, a tenant can choose to only have one VMs that is running the Seith engine, HIDS software as a sensor, and FW software as its executor. In addition, a tenant is not limited to single sensors and executors. In other word, a tenant can have multiple and different types of sensors and executors. For example, a tenant can scale its NIDS to multiple VMs to handle heavy network loads and all of them send their feedback to tenant's Seit Engine. Similarly, a tenant can scale his FW VMs (executors) and at the same time have an HAProxy (another executor) that load-balance the traffics among them. As long as Seit's interface is installed on the sensors and executors  there should be no limit on their numbers and verities. 
%
%\subsection{Reputation Manager (CM)}
%We can think of Reputation Manager as a tenant but with special features as following:
%\begin{itemize}
%\item \paragraphb{Initial Introducer} When the system boots up or new tenants join the system, they need an introducer to introduce them to other tenants since the system will not allow any communications without introduction. CM takes the responsibility to introduce when there is no chain of other tenants to reach the target tenant. This is also means that CM has a Seit Engine to receive and forward introduction request as other tenants do.
%
%\item \paragraphb{Services Tracker} Every tenant registers its services when it joins Seit system for the first time. Thus, if any tenant requests a certain service and it doesn't know its owner, it can request such information from CM.
%
%\item \paragraphb{Global Reputation Tracker}  Another important feature of CM is that it all other tenants in the system report to it of any certain behavior. Thus, CM keeps a centralized global reputation of all tenants and can make a wide view and central decisions (e.g. blocking or steering traffic of bad tenants). 
%
%
%\item \paragraphb{Introduction Chain Advertiser} In traditional IBR in P2P networks, nodes perform hill-climbing algorithm, where hosts advertise nodes they accept introductions from to other nodes. Instead, we make tenant advertise node the accept introduction to only CM where it can calculate the
%shortest/best path and return the paths to all tenants. We believe by involving CM in our system, we could save the tenants the extra overhead and delay caused by searching and discovering introduction path to destination (especially in large datacenters with thousands of tenants and services in it).
%\end{itemize}
%
%\subsection{Seit Messages}
%As shown in Figure \ref{fig:detailed-proc}, Seit framwork includes three type of messaging. Red arrows represent Inter-SeitEngine Messages, yellow arrows represent Tenant-CloudManager messages, and green arrows represent Tenant-Internal Messages. 
%
%\begin{itemize}
%\item \paragraphb{Inter-SeitEngine Messages} These messages are exchanged among Seit Engines that belong to different tenants. These messages are based on IBR reputation protocol. Seit is not tied to a specific reputation system. We are using IBR as it provides the local view where reputation
%is based on the perspective of the tenant receiving a reputation.
%
%\item \paragraphb{Tenant-CloudManager Messages} These messages are exchanged between Tenants and Reputation Manager.Such as registration request, service registration and introduction chain.
%
%\item \paragraphb {Tenant-Internal Messages} These messages are exchanged between Tenant's SE, Sensors, and Executors such as feedback from sensors to SE and actions from SE to executors 
%\end{itemize}
%
 %
%\subsection{Terminology}
%Before we start exploring Seit's  implementation details, it is important to understand and explain some terminology we use in Seit's framework. 
%\begin{itemize}
%\item \paragraphb{Feedback} Feedback could be internal (Sensor-Feedback), from tenant's own sensors, or external (Tenant-FeedBack), from other tenants. In the case of internal feedback, sensors send feedback, in a form of JSON message of {Tenant responsible, event triggered by this responsible tenant}, depend on their functionality. For example, Firewall sensors send feedback {Tenant X, authorized access to port 88}. In the case of external feedback, tenant receives feedback from Requester and Target Tenants in regards to the other end the tenant make the introduction for. For example in Figure , tenant B receives external feedback from A and C. 
%
%\item \paragraphb{Service Behavior} A tenant is responsible of its services and their behaviours when they interact with other tenants' services. Tenant's sensors notify SE with the behavior of other tenants' services and identify if the behaviour was negative or positive. Every tenant has his own definition of negative and positive behaviors. Negative behavior could be for example poor service provision or security violation. 
%
%\item \paragraphb{Tenant Reputation} (Need to rewrite this..) Every tenant within Seit's framework maintains two types of reputation: global and local. A global reputation that all other tenants contribute on building and is held by the Reputation Manager. It represents the reputation history of all tenant's connections. Local reputation, on the other hand, represents trust level for each tenant it has a connection with through introducers. Local reputation is asymmetric as two tenants can have different local reputation for each other.  For example in figure \ref{fig:IBR}, tenants B,C, and D all view the same global reputation of tenant A. at the same time, A's local reputation to B is different than to C and D. Every time two tenants establish a connection in Seit, both receive the tow reputations about the other. This gives both tenants the ability to make a broader decision and actions as we discuss on the next sections. 
%\end{itemize}

-------------------------------------
%%% FROM POLICIES and INTERFACES

%Policies for:
%1) When you'll make an introduction
%2) How to interpret negative/positive feedback from a given sensor.
%3) What action to take when a reputation changes (or is calculated for the first time)
  %-- part will be in Reputation Manager (when to notify), and part will be on each compone

%To make Seit fully integratable into cloud systems, we need two key
%interfaces: (i) interfaces between user components (\eg
%firewalls, load balancers, network controllers, etc.) and the
%reputation manager, and (ii) a configurable query interface that 
%allows configurable query mechanics and efficiently deals with the
%dynamics of a changing reputation graph.

%\subsubsection{Interfacing with Components}

%We classify cloud components into two types: sensors and actuators.
%These correlate with the two part of Seit's interface: reputation
%feedback and reputation querying. In reality, most components can
%implement both sensor and actuator interfaces.

----------------------------------------------------
%%% FROM IMPL.tex




%
%
%
%
%
%
%We have prototyped Seit on Linux systems with xxx and Mininet by following the architecture in Section \ref{sec:seit}. 
%It consists of approximately 7300 lines of Java code. 
%
%\subsection{Reputation Manager}
%Seit's Reputation Manager can potentially communicate with many tenants, each of which runs a small agent called the Seit Engine (SE). With this in mind, we implement the RM as a highly scalable Java-based server that uses Java NIO to efficiently handle a large number of tenant connections. We also provide an admin API to setup, install, and view policies across the cloud, as well as facilitate new tenants and their services. While the RM can be installed on any tenant or cloud server, we envision it as a centralized controller running as a service by the cloud provider to optimize the network (likely coupled with a hot-swappable backup server).
%
%\subsection{Seit Engine}
%The Seit Engine is a light weight Java process that can be installed on any tenant machine. It listens on two separate interfaces for internal and external communications. The internal interface is used to communicate with a tenant's own services, sensors, and executors, while the external interface is used to communicate with the RM. The SE can be configured with a text configuration file that specifies the following: 1) a list of components, each of which has the name of the component, IP, type (service, executor, sensor), component description and its tasks; 2) a threshold to block/refuse/accept connections from a tenant; 
%and (iii) the query rate limit.
%% the number of introductions to accept from an introducer.
%
%\subsection{Seit API}
%All communications in Seit are performed through Table~\ref{tab:api}'s set of API calls. These include 1) a registration request from sensors/executors to the RM when they boot up for the first time, 2) a connection request from a tenant's component, asking for a component (service) in another tenant, which is forwarded from the tenant's SE to the RM, 3) a feedback message containing the reputation score, and 4) a configuration message setting new thresholds or reputation scores.
%
%
%\begin{table}[t]
%\small
%\centering
%\begin{tabular}{|l|l|}
%\hline
%{\bf Functionality} & {\bf Seit API call}  \\
%\hline
%create a Seit API instance $s$ & {\tt s = create()}      \\
%\hline
%register a component $c$ & \multirow{2}{*}{{\tt res = register(s,c)}} \\ res = approved | denied  &     \\
%\hline
%send a connection request for $c$ & \multirow{2}{*}{{\tt res = request(s,c)} } \\ res = approved | denied &      \\
%\hline
%send reputation score $f$ to $c$  & {\tt feedback(s,c,f)}   \\
%\hline
%send config (or new score) $f$ to $c$  & {\tt config(s,c,f)}   \\
%\hline
%\end{tabular}
%\vspace{-0.1in}
%\caption{Seit's Application Programming Interface.}
%\label{tab:api}
%\end{table}
%
%%
%%\begin{itemize}
%%\item \paragraphb{RegistrationRequest} Sent from sensors and executors to JE when they boot up for the first time.
%%
%%\item \paragraphb{AccessServiceRequest} Sent from services within tenant's component to SE. When a service requests access to another services belong to another tenant, it must asks JE to establish the connection for it. JE then uses the Inter-SeitEngine Messages described above. 
%%
%%\item \paragraphb{ServiceAccessApproved} This is a reply to AccessServiceRequest message and sent from SE to a service requesting access to an external service. It is basically saying that connection is established and now services can communicate with each other.
%%
%%\item \paragraphb{ServiceAccessDenied} This is a reply to AccessServiceRequest message and Sent from SE to a service requesting access to an external service. This message can be either sent because SE receives IntroductionRefused or IntroductionDeclined as shown above.
%%
%%\item \paragraphb{SensorFeedback} Sent from tenant's sensors to its JE. The message includes providing SE with a score (to deduct or add) regarding the opposite sensor service's behavior. 
%%\end{itemize}
%%
%% In addition, we implemented Java package and classes that can be used to provide the essential classes the interfaces can be built from if the developer prefers Java to implement Seit's plugin.
%
%\subsection{Seit Shim Plugins}
%
%We provide a Seit plugin interface to easily accommodate shims for new components. This plugin provides two interfaces for a shim -- one for handling actions and the other for communicating and sending feedback to the SE. Users do not need to make any changes to the design and implementation of the components themselves, making it easier to deploy Seit on any infrastructure. For example, in order to use an HAProxy component in Seit, we map the commands received from the SE to HAProxy's actions, such as forwarding certain traffic to a certain destination, and provide an interface to report feedback scores to the SE. This process applies to sensors too; an IDS system such as Bro needs to send an alert for any security threads to Seit.    
%
%%We envision Seit's implementation to be appealing as it only requires implementing Seit Interface on the components that implement actions (executors) and the ones that send feedback to SE (sensors). With this approach, we don't need to make any changes to the design and implementation of the components themselves. Thus making Seit easy to implement at any infrastructure. For example, HAProxy developers do not need to change anything of the proxy's implementation. All what they need is to use Seit interface that opens a connection with the SE and maps the commands it receives from SE to the action that HAProxy normal does such as forward certain traffic to certain destination. Same thing with sensors. For example, IDS such as Bro only need to use the interface to send the alert for any security threats to SE. 
%
%% We tested the implementation of verity of plugin that use Seit's interface on the following multiple network and middlebox components:
 %
 %We have implemented the following proof of concept plugins to create shims for different types of components. We realize that there are various approaches to implement the plugins on each component but we provide our prototype to provide further understanding of the potential of Seit.
 %
 %\paragraphb{FloodLight plugin:} FloodLight is an SDN controller. The plugin maps the instructions received by the SE to OpenFlow rules and sends them through the FloodLight REST API to the controller. For example, if a tenant wants to terminate the connection established with another tenant, the tenant would send this information to Floodlight's Seit plugin interface, where it would be converted to an appropriate OpenFlow rule (using the two tenants' IPs). Our plugin would then insert this rule into the OpenFlow switches connecting these two tenants.
%
%
%\paragraphb{CloudFoundry plugin}
%Cloud Foundry (CF) developers interact with their services and search for other services provided in the "Marketplace" (a catalog of services and plans exposed to end users of a Cloud Foundry instance) through CF Command Line Interface (CLI). Marketplace services may come from one or many service brokers that advertise for these services. Cloud Foundry developers or admins can configure Seit's plugin to specify the threshold of service reputation they would like to allow their own services to interact with. The plugin invokes Cloud Foundry-CLI, filters, sort the marketplace results of the same service types (Database, Advertising, etc) based on their reputation.
 %
%\paragraphb{HAProxy plugin:} This plugin maps the instructions received by the Seit Engine to configurations written in a /haproxy.cfg file. For instance, in one use case a tenant would maintain two Web servers with the same URL, one to serve tenants with high reputation and the other for low reputation tenants. This tenant's SE then updates HAProxy with the other tenants' service IPs and reputations. 
%
%\paragraphb{Snort IDS plugin}
%Snort Intrusion Detection System provides the ability to log configured and specific alerts to Syslog where other programs (\eg SWATCH and Kiwi Syslog Daemon) can monitor the Syslog and take actions when they see the alert (\eg send an email to admin or start a third program). Our plugin takes advantage of these capabilities to send sensor feedback to Seit. We used SWATCH to monitor Syslog and launch Seit launch Seit's plugin and pass to it the alert it detected. Seit's plugin parses the alert and extracts information such as source IP and alert type and send the feedback to Seit with these information.
%
%\paragraphb{Nagios plugin:} An important and unique feature of Seit is the tenant's ability to police itself: the tenant can monitor the sentiment of other tenants (i.e., other tenants' opinions of itself) as discussed in Section \ref{sec:examples}. \fixme{(are ``sentiments'' here the same as reputations? --CJW) With Seit, the RM forwards tenants feedback about a service to the tenant that owns this service. We integrated this functionality by implementing a plugin within Nagios: an open source computer system monitoring, network monitoring and infrastructure monitoring software application. We took advantage of JNRPE (Java Nagios Remote Plugin Executor) to build a Java plugin that is listening for any sentiments sent by Seit's Reputation Manager. In our implementation test setup we have tenant-3 communicating with tenant-1, tenant-2, and tenant-4.  Nagios server is running on a machine belongs to tenant-3. When tenant-1, tenant-2 and/or tenant-4 complain to Seit about tenant-3. They send their updated tenant-3 reputation to Seit's Reputation Manager who forwards this feedback to tenant-3. Figure \ref{fig:nagiousPlugin} shows Seit's plugin in Nagios where we call it SEIT-CHECK Tenant-3 can setup Nagios with any threshold and warnings he wants. For now, "Warning" alert if its reputation to a tenant falls below 0.5. "Critical" alert if its reputation to a tenant falls below 0.2.}
%
%%\begin{figure}
%%\centering
%%\includegraphics[width =\columnwidth]{graphs/seit-plugin-description}
%%\caption{Seit's plugin in Nagios}
%%\label{fig:nagiousPlugin}
%%\end{figure}
%
%
%
%
%%
%%Implementation is based on two levels, Infrastructure as a Service (IaaS) and Platform as a Service (PaaS). In IaaS, actions are mostly applied by Reputation Manager as they are highly coupled with the infrastructures. For example, tenants inform Reputation Manager of the traffic they want to accept. Accordingly, Reputation Manager control the traffic and steer it by inserting OpenFlow rules on the tenants' switches.  Another example is launching tenant's VM based on its reputation. Tenant in OpenStack for example can choose, if they have the authority, to launch their VMs and services in the hardware they choose. For that, a tenant that provide a database service can choose on which server trusted tenants should have their accounts. Thus, mimizing the risk of mixing them with untrusted tenants accounts.   \paragraphb{Talk more and in detail about CM interface with OF}
%%
%%PaaS on the other hand gives another level of control for tenants that do not have the authority and control over the infrastructure.  An example can be seen in CloudFoundry platform where it laucnh VM services such as HAProxy, Router, and Container for developers and loadbalance and control the traffic among the developer's VM such as Web services. Seit can be used here to instruct certain actions on HAProxy to forward traffic to specific destinations based on trust level of the source.  
%
%
%%
%%
%%In this section the messages that comprise Seit system are enumerated, with a brief explanation of their purpose.
%%We could envision a high level view of Seit as shown in Figure \ref{fig:Seit-high-level}
%%\begin{figure*}
%%		\centering
%%        \includegraphics[width=\textwidth]{graphs/Seit-High-level.pdf}
%%        \caption{Seit High Level}
%%        \label{fig:Seit-high-level}
%%\end{figure*}
%%
%%\subsubsection{Inter-SeitEngine Messages}
%%\footnote{Most of the Inter-Tenants messages and their explanations are copied from IBR specification with some modifications and addition to meet Seit's requirements}. Figure \ref{fig:intro-process} highlights the initial request and offer messages among Requester, Introducer and Target tenants.
%%
%%\begin{figure}[t]
%%		\centering
%%        \includegraphics[width=\columnwidth]{graphs/IBR-Seit.pdf}
%%        \caption{Introduction Process}
%%        \label{fig:intro-process}
%%\end{figure}
%%
%%\begin{itemize}
%%\item \paragraphb{IntroductionRequest} Sent from the Requester to the Introducer, asking the Introducer to perform an introduction.
%%
%%\item \paragraphb{IntroductionDenied} Sent from the Introducer to the Requester, in response to an IntroductionRequest, indicating an inability or a refusal to perform the requested introduction.
%%
%%\item \paragraphb{IntroductionOffer} Sent from the Introducer to the Target in response to an IntroductionRequest. This message includes Introducer's Trust Level to Requester. 
%%
%%\item \paragraphb{IntroductionDeclined} Sent by the Target to the Introducer in response to an IntroductionOffer. Indicates an unwillingness to accept the introduction.
%%
%%\item \paragraphb{IntroductionRefused} Sent by the Introducer in response to an IntroductionDeclined message to Requester, letting the Requester know that the introduction was refused. 
%%
%%\item \paragraphb{IntroductionAccepted} Sent by the Target to the Introducer, indicating acceptance of the introduction. This message includes keying material and configuration information needed by the other party (Target or Requester) in order to establish the connection.
%%
%%\item \paragraphb{ConnectionEstablished} Sent by the Introducer to the Requester iff the Target sent IntroductionAccepted messages. This message includes Introducer's Trust Level to Target. This message tells the Requester that the Target has accepted the introduction and conveys the configuration information and keying material that the other party provided.
%%
%%\item \paragraphb{TenantFeedback} Sent by the Requester and the Target to the Introducer, providing the Introducer with a binary feedback regarding the opposite party’s behavior. Feedback has a Reporter (the tenant that initiated the feedback), a Subject (the tenant at the other end of the connection whose behavior is being reported on), and a binary score (0 or 1) to indicate if it is a negative or positive feedback. 
%%
%%\item \paragraphb{CloseConnection}  When a participant closes a connection, it should send a CloseConnection message. (Without a CloseConnection message, 
%%the other participant will not close its side of the connection 
%%until it times out waiting to receive Hello messages.) CloseConnection message is sent by a tenant to its pier when the tenant's Trust Level to its pier reaches its threshold or the connection is timed out because no further Hello messages were received in a certain amount of time. 
%%
%%
%%\subsubsection{Tenant-CloudManager Messages}
%%\begin{itemize}
%%\item \paragraphb{RegisterationRequest} Sent from Tenant to CloudManager when the Tenant joins Seit network for the first time. The message contains Tenant's ID, Tenant JE's IP, and Tenant's provided services.
%%
%%\item \paragraphb{AcceptIntroducer} Sent from Tenant to CloudManager to indicate the acceptance of introductions from another tenant. CloudManager uses this information to build the Introduction chain and send the chain to all tenants in the network. 
%%
%%\end{itemize}
%%
%%\subsubsection{Tenant-Internal Messages}
%%


==> overview.tex <==
%\section{Overview}
%
%\eric{WE SHOULD REMOVE THIS SECTION}
%
%Our goal in this project is to address the challenges
%from the previous section without affecting the performance or the quality of service of tenants' applications. Our solution, Seit, provides an automotive high efficient system that gives each tenant the ability to classify other tenants based on their reputations and apply the corresponding actions. Seit provides an automatic system to dynamically manage and control inter-tenant communications in two steps (Automatic Tenant Classification followed by Automatic Differentiate Actions) as described next.
%
%\subsection{Automatic Tenant Classification}
%To accomplish automatic tenant classification, Joober implements a modified approach of Introduction Based Routing (IBR) protocol used in P2P systems. With IBR, peers are giving the choices with whom they interact with by providing incorporating feedback, giving participants a basis for making their relationship choices. IBR is decentralized system and requires minimum information sharing among peers and designed to scale to Internet sized networks with no modifications to operating systems and network backbone. To better understand IBR, consider the following example showing in Figure \ref{fig:IBR}
%
%\begin{figure}[t]
		%\centering
        %\includegraphics[width=\columnwidth]{graphs/IBR.pdf}
        %\caption{IBR}
        %\label{fig:IBR}
%\end{figure}
%
%Nodes A, B, C and D are peers in P2P system. The
%green lines indicate established connections. Each node
%maintains reputation score (trust level) for the nodes connected to
%it. When Node A wants to communicate with D, it
%must follow the chain of connections between it and D
%and ask the nodes in the chain for introduction to the
%node after. A starts asking B for introduction to C.
%Node B looks at nodes A behavior history (represented
%by reputation score AB) and decides whether or not to
%forward A's request to C. If the request is forwarded, C
%looks at behavior history of B (BC) and decides whether
%or not to accept the introduction request. The process
%continues until A reaches D. If B, C, or D rejects a request, node A will not be able to communicate with D. After the connection is established between A and C, C assigns a reputations score to A (CA) which is X*BC. Same thing with D where it assigns reputations
%score of DA which is X* DC. If A starts behaving negatively
%(e.g. sending malicious packets to D), D will decrease
%A's score DA and also decreases C's score DC since C
%took the responsibility and introduced A to D. C will
%do the same and decrease A's score AC and B's score
%since it introduced A to C. And finally, B will decrease
%As reputation score AB. By this approach, nodes take
%extra cautious of whom they introduce and eventually,
%bad behaving nodes will be left alone with no other
%nodes willing to introduce them when their scores fall
%under the minimum trust level score.
%
%In Seit, we used the same approach but on a tenant level. Tenants are giving the choice of whom to communicate with and can start connections through introductions and based on their behaviors (need to show example or use case of such interaction e.g web with Ad or database service??). Since tenants own and provide more than one service, they are responsible for their services behaviors and any miss behaving service will affect the tenants reputation. Moreover, although we could make Seits
%reputation system be completely decentralized, we decided to take advantage of the existing of a centralized management entity in the cloud to better provide IBR system with more robust implementation. When tenants detect negative behaviors, not only they will make decision of future introduction acceptance, but also inform
%the Cloud Manage CM of these behaviors. This information helps CM to get a wide view of his datacenter and tenant sharing its resources and their overall behaviors which lead to make valuable decisions applied
%to tenant (isolating bad tenants, blocking their traffic, etc.).
%
%
%\subsection{Automatic Traffic Differentiate Actions}
%Once tenants are classified based on their behaviors, a tenant could easily differentiate set of actions for each class of tenants its communicating with. 
%An example of such action is applying SDN. When one of the tenants
%service (source) starts communicating with a service (destination) that belongs to another tenant (after introduction), Seit looks at sources reputation score and
%matches the routing decision for destination (e.g steer the traffic to go through security MBs). Right after that, Seit informs the Openflow
%controller with these information (source IP, destination IP, protocol, action, etc.) so the controller can apply the appropriate rule for the traffic between the
%two services. 
%
%
%\begin{figure}[t]
		%\centering
        %\includegraphics[width=\columnwidth]{graphs/Seit-components.pdf}
        %\caption{Seit Architecture}
        %\label{fig:detailed-proc}
%\end{figure}
%

